Haptics of Screwing and Unscrewing for its Application in Smart Factories for Disassembly

Reconstruction of skilled humans sensation and control system often leads to a development of robust control for the robots. We are developing an unscrewing robot for the automated disassembly which requires a comprehensive control system, but unscrewing experiments with robots are often limited to several conditions. On the contrary, humans typically have a broad range of screwing experiences and sensations throughout their lives, and we conducted an experiment to find these haptic patterns. Results show that people apply axial force to the screws to avoid screwdriver slippage (cam-outs), which is one of the key problems during screwing and unscrewing, and this axial force is proportional to the torque which is required for screwing. We have found that type of the screw head influences the amount of axial force applied. Using this knowledge an unscrewing robot for the smart disassembly factory RecyBot is developed, and experiments confirm the optimality of the strategy, used by humans. Finally, a methodology for robust unscrewing algorithm design is presented as a generalization of the findings. It can seriously speed up the development of the screwing and unscrewing robots and tools.

==> ieeepreamble.tex <==
%% %%%%%%%%%%%%%%%%%%%%%%%
%% Packages to be used
%% %%%%%%%%%%%%%%%%%%%%%%%
\pdfminorversion=4
\usepackage{microtype}
\usepackage{cmap} %make russian copiable in pdf
%\usepackage[T1,T2A]{fontenc}
%\usepackage{lmodern}
% \usepackage[utf8]{inputenc}%включаем свою кодировку: koi8-r или utf8 в UNIX, cp1251 в Windows
% \usepackage[english]{babel}
% \usepackage{amssymb,amsfonts,amsmath,mathtext,enumerate,float} %подключаем нужные пакеты расширений %removed cite
% \usepackage{lineno}  % for line numbering during review
%\linenumbers

%%All the packages from the template
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed

\usepackage{xspace} % To avoid problems with missing or double spaces after
                    % predefined symbold
% \usepackage{caption} %these three command get the figure and table captions automatically small
% \renewcommand{\captionfont}{\small}
% \renewcommand{\captionlabelfont}{\small}
% \usepackage{subcaption}
% \usepackage{tabularx} %to be able to use multiline tables

%% Graphics
\usepackage{graphicx}  % to include figures (can also use other packages)
% \usepackage{color}
% \usepackage{colortbl}
% \usepackage{rotating}
\graphicspath{{./pics/}} % Make Latex search fig subdir for figures
\DeclareGraphicsExtensions{%
    .png,.PNG,%
    .pdf,.PDF,%
    .jpg,.mps,.jpeg,.jbig2,.jb2,.JPG,.JPEG,.JBIG2,.JB2}

%% Math
\usepackage{upgreek} % Adds in support for greek letters in roman typeset

% \usepackage{multirow}
%\usepackage{rotating}

% \newcommand{\rotatedHead}[1]{\rotatebox{60}{\parbox{5cm}{#1}} }

%% fix to allow peaceful coexistence of line numbering and
%% mathematical objects
%% http://www.latex-community.org/forum/vbibiewtopic.php?f=5&t=163
%%
% \newcommand*\patchAmsMathEnvironmentForLineno[1]{%
% \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
% \expandafter\let\csname oldend#1\expandafter\endcsname\csname
% end#1\endcsname
%  \renewenvironment{#1}%
%    {\linenomath\csname old#1\endcsname}%
%    {\csname oldend#1\endcsname\endlinenomath}%
% }
% \newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
%   \patchAmsMathEnvironmentForLineno{#1}%
%   \patchAmsMathEnvironmentForLineno{#1*}%
% }
% \AtBeginDocument{%
% \patchBothAmsMathEnvironmentsForLineno{equation}%
% \patchBothAmsMathEnvironmentsForLineno{align}%
% \patchBothAmsMathEnvironmentsForLineno{flalign}%
% \patchBothAmsMathEnvironmentsForLineno{alignat}%
% \patchBothAmsMathEnvironmentsForLineno{gather}%
% \patchBothAmsMathEnvironmentsForLineno{multline}%
% }
%
%
% \newcommand{\tis}     {\ensuremath{\mathrm{TIS}}}
% \newcommand{\nottis}  {\ensuremath{\overline{\mathrm{TIS}}}}
% \newcommand{\tos}     {\ensuremath{\mathrm{TOS}}}
% \newcommand{\nottos}  {\ensuremath{\overline{\mathrm{TOS}}}}

% \usepackage[backend=biber,sorting=none,style=IEEEtranS]{biblatex}
% \bibliographystyle{IEEEtranS}
% \bibliography{IEEEabrv,Skoltech}


%\usepackage{geometry} % Меняем поля страницы
%\geometry{left=2.5cm}% левое поле
%\geometry{right=1.4cm}% правое поле
%\geometry{top=1.7cm}% верхнее поле
%\geometry{bottom=1.7cm}% нижнее поле

\usepackage[nodisplayskipstretch]{setspace}


\usepackage[font=footnotesize]{caption}
\usepackage[font=footnotesize]{subcaption}

% Get hyperlinks to captions and in references.
% These do not work with revtex. Use "hypertext" as class option instead.
% \usepackage{hyperref}    % Hyperlinks in references
% \usepackage[all]{hypcap} % Internal hyperlinks to floats.
\usepackage{bookmark}


% Make this the last packages you include before the \begin{document}
%\usepackage{cite} % Allows for ranges in citations
%\usepackage{mciteplus}

\newcommand{\TODO}[1]{{\LARGE TODODODO:} \textcolor{red}{#1}}
\newcommand{\exTODO}[1]{}
\newcommand{\code}[1]{\texttt{#1}}

% paragpaph titles in bold
% \usepackage{titlesec}
% \titleformat{\paragraph}[runin]
% {\bfseries\scshape}{\theparagraph}{1em}{}
% \makeatletter
% \renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
%                                     {3.25ex \@plus1ex \@minus.2ex}%
%                                     {-1em}%
%                                     {\normalfont\normalsize\bf}}
%
% \makeatother

\usepackage{listings}
\usepackage{color}

% \definecolor{mygreen}{rgb}{0,0.6,0}
% \definecolor{mygray}{rgb}{0.5,0.5,0.5}
% \definecolor{mymauve}{rgb}{0.58,0,0.82}
%
% \lstset{ %
%   backgroundcolor=\color{white},   % choose the background color
%   basicstyle=\footnotesize,        % size of fonts used for the code
%   breaklines=true,                 % automatic line breaking only at whitespace
%   captionpos=b,                    % sets the caption-position to bottom
%   commentstyle=\color{mygreen},    % comment style
%   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
%   keywordstyle=\color{blue},       % keyword style
%   stringstyle=\color{mymauve},     % string literal style
% }

%%
%% Julia definition (c) 2014 Jubobs
%%
% \lstdefinelanguage{Julia}%
%   {morekeywords={abstract,break,case,catch,const,continue,do,else,elseif,%
%       end,export,false,for,function,immutable,import,importall,if,in,%
%       macro,module,otherwise,quote,return,switch,true,try,type,typealias,%
%       using,while},%
%    sensitive=true,%
%    alsoother={$},%
%    morecomment=[l]\#,%
%    morecomment=[n]{\#=}{=\#},%
%    morestring=[s]{"}{"},%
%    morestring=[m]{'}{'},%
% }[keywords,comments,strings]%
%
% \lstset{%
%     language         = Julia,
%     basicstyle       = \ttfamily,
%     keywordstyle     = \bfseries\color{blue},
%     stringstyle      = \color{magenta},
%     commentstyle     = \color{ForestGreen},
%     showstringspaces = false,
% }
%
% \lstset{%
%     tabsize = 2,
% }


==> rtos_comparison_tabular.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline
RTOS feature & eCos & uc/OS-II & scmRTOS & freeRTOS \\ \hline
Free of charge & +/- & - & + & + \\ \hline
Open-source & + & + & + & + \\ \hline
Required functions support & +++ & ++ & + & ++ \\ \hline
Port for STM & +/- & + & + & + \\ \hline
Small footprint size & ++ & + (5-24KB) & +++ ($\sim 2$ KB) & ++ (5-10KB) \\ \hline
Different architecture support & ++ & +++ & ++ & +++ \\ \hline
Context switching speed & ? & ? & ++ ($1-2 \mu \textrm{s}$) & +++ ($\sim 1 \mu \textrm{s}$) \\ \hline
Number of processes & ? & ++ (250) & + (31) & +++ (limited by RAM) \\ \hline
Documentation quality, availability of examples & + & + & +++ & +++ \\ \hline
\end{tabular}


==> screw_recognition_tabular.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline &
\bf {Train IoU, \%} &
\bf {Validation IoU, \%} &
\bf {Forward time, ms } &
\bf {Screws detected, \%}
%\bf \shortstack{Screws detected,\\controlled conditions, \%}
\\
\hline
\bf SSD &
63.05 &
61.42 &
1450 &
-\\
\hline
\bf UNet &
66.12 &
64.42 &
2700 &
60 \\
\hline
\bf SegNet &
48.39 &
40.66 &
850 &
61\\
\hline
\bf SegNet + HN$^*$ &
67.95 &
66.08 &
850 &
63\\
\hline
\bf \shortstack{SegNet + HN$^*$ + WL$^{**}$} &
68.44 &
66.83 &
850 &
62\\
\hline
\end{tabular}

